Least Square Calibration for Peer Review

Peer review systems such as conference paper review often suffer from the issue of miscalibration. Previous works on peer review calibration usually only use the ordinal information or assume simplistic reviewer scoring functions such as linear functions. In practice, applications like academic conferences often rely on manual methods, such as open discussions, to mitigate miscalibration. It remains an important question to develop algorithms that can handle different types of miscalibrations based on available prior knowledge. In this paper, we propose a flexible framework, namely least square calibration (LSC), for selecting top candidates from peer ratings. Our framework provably performs perfect calibration from noiseless linear scoring functions under mild assumptions, yet also provides competitive calibration results when the scoring function is from broader classes beyond linear functions and with arbitrary noise. On our synthetic dataset, we empirically demonstrate that our algorithm consistently outperforms the baseline which select top papers based on the highest average ratings.

==> tmp_sijun.tex <==
\paragraph{Experiment Setup} Our experiments have two settings. In the first setting, all reviewers' scoring functions are linear. In the second setting, the scoring functions consist of $50\%$ arbitrary monotonic increasing function, $25\%$ convex functions, and $25\%$ concave functions. For each setting,  we consider 4 hyperparameters in our experiments: The number of papers $N$, number of reviewers $M$, the number of papers $k$ that each reviewer reviews, as well as the standard deviation of noise $\sigma$. We use $N = 1000, M=1000, k=5, \sigma=0$ as our baseline noiseless setting, and $\sigma=0.5$ as our baseline noisy setting. For each set of hyperparameter, the reported results are averaged over 20 trials. All of our models are implemented with the Gurobi Optimizer~\cite{gurobi}.

\paragraph{Dataset Generation} We sample each paper's true quality from a Gaussian distribution $x \sim \N(5, 1.6)$, and truncate the value to be within the $[0,10]$. Our assignment algorithm ensures that the majority of papers will get reviewed by exactly $k$ reviews. (assuming $N = M$). Each reviewer is randomly assigned scoring function. Before applying the scoring function, a zero-mean Gaussian error $\epsilon \sim \N(0, \sigma)$ is added to the true qualities for each reviewer-paper pair. We leave the details of how we generate our scoring functions as well as the assignment algorithm to the Appendix.




==> xiaohui.tex <==
% !TEX root = main.tex

\subsection{Linear Scoring Functions with No Noise}
Going beyond monotonicity, next we investigate the scenario where the reviewers' scoring functions are linear functions and there is no  noise added to them. In this case,   we can add a set of \textit{linear equality constraints} to the system and obtain a feasibility linear program:

% \begin{align}\label{lp:linear}
% 	&\min 1 \\
% 	&\textup{s.t} \nonumber\\
% 	&x(I^\ell_j) - x(I_j^{\ell-1}) \geq 1 \quad \forall j \in [M], \forall 2 \leq \ell \leq |I_j| \nonumber \\
% 	&\frac{x(I^\ell_j) - x(I_j^{\ell-1})}{y^\ell_j - y^{\ell-1}_j} = \frac{x(I^{\ell+1}_j) - x(I_j^{l})}{y^{\ell+1}_j - y^{\ell}_j} \quad \forall j \in [M], \forall 2 \leq \ell \leq |I_j| \nonumber
% \end{align}
\vspace{3pt}
\hrule
\vspace{1pt}
\noindent\textbf{\LSC with linear scoring functions and no noise}
\begin{align}\label{lp:linear}
    \min_{\mathbf{x}, \mathbf{\epsilon}} & \quad 0 \\ \nonumber
	\textup{s.t. }&\quad x(I_j^\ell) - x(I_j^{\ell-1}) \geq 1 \tag*{$\forall j \in [M], \forall 2 \leq \ell \leq |I_j|$} \\\nonumber
	&\quad \frac{x(I_j^\ell) - x(I_j^{\ell-1})}{y^\ell_j - y_{j}^{\ell-1}} = \frac{x(I_j^{\ell+1}) - x(I_j^{\ell})}{y_{j}^{\ell+1} - y_{j}^{\ell}} \\  \nonumber
    & \tag*{$\forall j \in [M], 2 \leq \ell \leq |I_j| -1 $}
\end{align}
\hrule
\vspace{1pt}

\jw{Here to guarantee $x(I_j^\ell)$ to be strictly larger than $x(I_j^{\ell-1})$ and we w.l.o.g. use $\geq 1$ for convenience since rescaling the solution will not change ranking.}

With the prior knowledge that the scoring functions are all linear functions and that there is no noise, it is easy to see that the true item qualities $\mathbf{x}^*$ and scoring functions $\mathbf{f}^*$ must be a feasible solution to this program. However, we cannot guarantee that LP~\eqref{lp:linear} does not have any other feasible solutions whose induced item order disagrees with $\mathbf{x}^*$.
This could happen, for example, when the reviewers do not review enough items, or their assigned items do not have enough overlap to perform a full calibration.
Therefore, it remains an important question that under what condition   we can  (essentially) perfectly recover  all item qualities using LP~\eqref{lp:linear}, in the following sense.

\begin{definition}[Perfect Recovery]
	A set of qualities $\{x(i)\}_{i \in [N]}$ is said to \emph{perfectly recover} the true qualities $\{x^*(i)\}_{i \in [N]}$ if there exists $a > 0$ and $b$ such that $x(i) = ax^*(i)+b$ for every $i \in [N]$.
\end{definition}

We remark that perfect recovery is a stronger condition than   recovering just the \emph{correct order} of the items. It additionally requires that the  quality gaps among different items are proportional to the gaps of true qualities. 

One might wonder whether such a strong goal of perfect recovery may be too good to be possible. Surprisingly, our next result formally show that if the reviewer assignments satisfy some reasonable constraints, it is indeed possible to hope for perfect recovery. To introduce our result, we introduce a novel notion of a \textit{review graph} and its \emph{recover-robustness}.  The review graph is a graph that connects reviewers to each other according to the number of common items that they reviewed.

 

	\begin{definition}[Review Graph and  Recovery-Robustness] \label{def:review-graph}
	A \emph{review graph} is an undirected multi-graph\footnote{A multi-graph is a graph that allows multiple edges between two vertices.} $G=(V,E)$ where $V$ is the set of reviewers, and there are $|I_i \intersect I_j|$ edges connecting every two reviewers $i, j \in V$. A review graph $G$ is said to be  \emph{recovery-robust} if for any item assignments inducing $G$ and any   given review scores  $\{y_j^l \}_{j,l}$, any solution to LP \eqref{lp:linear} is a perfect recovery. 
\end{definition} 

Interestingly,  it turns out that the recovery-robustness of a review graph is fully characterized by a novel notion of \emph{graph connectivity}, which we now introduce. A connected component of the reviewer graph is simply a subset of reviewers $S \subseteq [M]$ who connects to each other. We will refer to the items they have collectively reviewed, $C(S) = \bigcup_{i\in S} I_i$, as the items \emph{covered} by component $S$.  We next introduce   \emph{double connectivity}, which naturally generalizes graph connectivity.
% , which is a sub-graph with min cut at least $1$.


The (standard) components of a graph can be identified through a \texttt{Repeat-Union} procedure, where we start by treating each node as a component and then repeatedly joining two components whenever they share at least \emph{one} edge. Our notion of    \emph{doubly-connected component} include all components that can be found using the same joining procedure, except that each time we join two components only when they share at least \emph{two} edges. A formal procedure, coined \texttt{Repeat-Union2}, is given in Algorithm \ref{alg:union}.

\begin{algorithm}[ht]
	\caption{\texttt{Repeat-Union2}}
	\label{alg:union}
	\begin{algorithmic}[1]
		\INPUT review graph with $N$ item, $M$ reviewer, and item assignment set $\{I_j\}_{j\in [M]}$
		\STATE $U \leftarrow \{\{1\}, \{2\}, \ldots, \{M\}\}$
		\WHILE {$\exists S_1, S_2 \in U$, s.t. $|C(S_1) \cap C(S_2)| \geq 2$ }
		\STATE $U \leftarrow U - S_1 - S_2 + (S_1 \cup S_2)$ (i.e., merge $S_1, S_2$)
		\ENDWHILE
		%		\IF {there exists $S \in U$ such that $C(S) = [N]$}
		%		\STATE return YES
		%		\ELSE
		\STATE \textbf{return} $U$
		%		\ENDIF
		% \STATE return $\algorithmicfalse$
	\end{algorithmic}
\end{algorithm}



\begin{definition}[Doubly-connected component] \label{def:double-connect}
Any component returned by Algorithm \ref{alg:union} is called a \emph{doubly-connected component}.
\end{definition}


The following theorem shows that to guarantee perfectly recovered qualities from LP \eqref{lp:linear} under linear scoring functions without noise, it is necessary and sufficient to have  a \emph{doubly-connected} component that covers all items.  

\begin{theorem}\label{thm:perfect}
	A review graph $G$ is   recovery-robust \emph{if and only if }   the review graph $G$ has a doubly-connected component $S$ that covers all items, i.e. $C(S) = [N]$.  
\end{theorem} 
 
Below we show a proof sketch of the doubly-connected component part. Please see appendix for the full proof. Whenever there are two reviewers $j_1$ and $j_2$ with $|I_{j_1} \cap I_{j_2}| \geq 2$, we can use the scores they give to these common items to calibrate ``locally'' between these two reviewers, such that after the calibration, we can merge them into a single reviewer who reviews all the items $I_{j_1} \cup I_{j_2}$. Algorithm~\ref{alg:union} follows exactly this idea by repeatly merging two reviewers into a single review, until there is some reviewer with whom we have the review scores to the entire item set $[N]$, and these are the calibrated qualities that we want. 

For the reverse direction, we could exhaustively merge all doubly-connected components according to Algorithm~\ref{alg:union}, such that the remaining graph must have at most one edge between any two vertices. Suppose the true quality $x^*_e$ of the item that corresponds to the edge $e=(i,j)$ has the form of $-\sqrt{p_i}-\sqrt{p_j}$, where we let $p_i$ be the $i$th smallest prime number. We can show that no two items would share the same quality. In addition, there exists a transform with $k_i=\sqrt{p_i}, b_i=p_i$ such that $\widetilde x_e = k_i x_e+b_i=k_j x_e+b_j$ is also a valid solution to LP~\eqref{lp:linear}. In particular, as we set $k_i\neq k_j$, such transformation on the vector of true qualities is non-linear, and therefore implies the graph is not recovery-robust.  
 
  

\noindent {\bf Remark:} Theorem \ref{thm:perfect} also provides useful insights for reviewer assignment in applications. Specifically, it appears that having stronger connection among reviewer during review assignment, defined formally in the sense of   Definition \ref{def:double-connect} and its generalizations, will be more helpful to calibrate their reviews.

